Generative Artificial Intelligence in Robotic Manipulation: A Survey

This survey provides a comprehensive review on recent advancements of generative learning models in robotic manipulation, addressing key challenges in the field. Robotic manipulation faces critical bottlenecks, including significant challenges in insufficient data and inefficient data acquisition, long-horizon and complex task planning, and the multi-modality reasoning ability for robust policy learning performance across diverse environments. To tackle these challenges, this survey introduces several generative model paradigms, including Generative Adversarial Networks (GANs), Variational Autoencoders (VAEs), diffusion models, probabilistic flow models, and autoregressive models, highlighting their strengths and limitations. The applications of these models are categorized into three hierarchical layers: the Foundation Layer, focusing on data generation and reward generation; the Intermediate Layer, covering language, code, visual, and state generation; and the Policy Layer, emphasizing grasp generation and trajectory generation. Each layer is explored in detail, along with notable works that have advanced the state of the art. Finally, the survey outlines future research directions and challenges, emphasizing the need for improved efficiency in data utilization, better handling of long-horizon tasks, and enhanced generalization across diverse robotic scenarios. All the related resources, including research papers, open-source data, and projects, are collected for the community in https://github.com/GAI4Manipulation/AwesomeGAIManipulation

==> sections/tax_test.tex <==
\begin{figure*}[!t]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\small,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            [
                {Generative Models for Robotic Manipulation}
                , ver, 
                color=hidden-draw, fill=mygray!100, 
                text width=22em, 
                text=black
                [
                    Foundation Layer (\S 2.1), fill=myred!80, text width=12em, text=black
                    [
                        Data Generation (\S 2.1.1), fill=myred!60, text width=14em, text=black
                        [
                            Data Generation via Simulation \\
                            Data Generation via Generative Model \\
                            Data Augmentation using Generative Model
                            , color=hidden-draw, fill=myred!40, text width=23em, text=black
                        ]
                    ]
                    [
                        Reward Generation (\S 2.1.2), fill=myred!60, text width=14em, text=black
                        [
                            Supervision signal\\
                            Policy score
                            , color=hidden-draw, fill=myred!40, text width=23em, text=black
                        ]
                    ]
                ]
                [
                   Intermediate Layer (\S 2.2), fill=myblue!80, text width=12em, text=black
                       [
                             Natural Language Generation (\S 2.2.1), fill=myblue!60, text width=14em, text=black
                             [
                                Natural Language Generation for Task Decomposition \\ Translated GPT~\cite{huang2022language}, Embodied Agent~\cite{li2024embodied}\\
                                Physically-Grounded Natural Language Generation \\
                                Natural Language Generation with External Memory \\
                                Action Generation with Natural Language Generation, color=hidden-draw, fill=myblue!40, text width=23em, text=black
                             ]
                       ]
                       [
                           Code Generation (\S 2.2.2), fill=myblue!60, text width=14em, text=black 
                           [
                                Direct Code Generation  \\
                                Decomposition-based Generation \\
                                Constraint-based Generation 
                                , color=hidden-draw, fill=myblue!40, text width=23em, text=black
                           ]
                       ]
                       [
                              Visual Generation (\S 2.2.3), fill=myblue!60, text width=14em, text=black
                              [
                                Video Generation Models \\
                                Image Generation Models
                                , color=hidden-draw, fill=myblue!40, text width=23em, text=black
                              ]
                       ]
                       [
                           State Generation (\S 2.2.4), fill=myblue!60, text width=14em, text=black
                           [
                               Visual State \\
                                Action State
                                , color=hidden-draw, fill=myblue!40, text width=23em, text=black
                           ]
                       ]
                ]
                [
                   Policy Layer (\S 2.3), fill=myyellow!80, text width=12em, text=black
                       [
                             Grasp Generation (\S 2.3.1), fill=myyellow!60, text width=14em, text=black
                             [
                                Diffusion-based generation \\
                                Other generative models 
                                , color=hidden-draw, fill=myyellow!40, text width=23em, text=black
                             ]
                       ]
                       [
                             Trajectory Generation (\S 2.3.2), fill=myyellow!60, text width=14em, text=black
                             [
                                Latent Space Generation \\
                                Sampling-based Generation \\
                                Hybrid-mode Generation 
                                , color=hidden-draw, fill=myyellow!40, text width=23em, text=black
                             ]
                       ]
                ]
            ]   
        \end{forest}
    }
    \caption{Overview of generative models for robotic manipulation. The taxonomy shows three main categories, each with detailed sub-categories describing specific approaches and methodologies in robotic manipulation.}
    \label{fig:taxonomy}
\end{figure*}

==> sections/taxonomy.tex <==
\begin{figure*}[!t]
    \centering
    \resizebox{\textwidth}{!}
    
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\small,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            [
                {Generative Models for Robotic Manipulation}
                , ver, 
                color=hidden-draw, fill=mygray!100, 
                text width=22em, 
                text=black
                [
                    Foundation Layer (\S 2.1), fill=myred!80, text width=10em, text=black
                    [
                        Data Generation (\S 2.1.1), fill=myred!60, text width=14em, text=black
                        [
                            {Data Generation via Simulation \\
                            }, color=hidden-draw, fill=myred!40, text width=23em, text=black
                        ]
                        [
                            {Data Generation via Generative Model \\
                            }, color=hidden-draw, fill=myred!40, text width=23em, text=black
                        ]
                        [
                            {Data Augmentation using Generative Model \\
                            }, color=hidden-draw, fill=myred!40, text width=23em, text=black
                        ]
                    ]
                    [
                        Reward Generation (\S 2.1.2), fill=myred!60, text width=14em, text=black
                        [
                            {Providing Supervision with Generative Model\\
                            }, color=hidden-draw, fill=myred!40, text width=23em, text=black
                        ]
                        [
                            {Providing Policy Scores with Generative Model\\
                            }, color=hidden-draw, fill=myred!40, text width=23em, text=black
                        ]
                    ]
                ]
                [
                   Intermediate Layer (\S 2.2), fill=myblue!80, text width=10em, text=black
                       [
                             Natural Language Generation (\S 2.2.1), fill=myblue!60, text width=14em, text=black
                             [
                                {Natural Language Generation for Task Decomposition \\
                                % \textit {\footnotesize{e.g., Translated GPT~\cite{huang2022language}, Embodied Agent~\cite{li2024embodied}, EmbodiedGPT~\cite{mu2024embodiedgpt},}} \\ \textit 
                                % {\footnotesize{Matcha~\cite{zhao2023chat}, DEDER~\cite{choiembodied}}}
                                } , color=hidden-draw, fill=myblue!40, text width=23em, text=black  
                             ]
                             [
                                {Physically-Grounded Natural Language Generation \\
                                % \textit {\footnotesize{e.g., SayCan~\cite{Ahn2022DoAsICan}, Grounded Decoding~\cite{huang2024grounded}, 
                                % Monologue~\cite{huang2022inner}, PhyGrasp~\cite{guo2024phygrasp}}}
                                }, color=hidden-draw, fill=myblue!40, text width=23em, text=black 
                             ]

                             [
                              {Natural Language Generation with External Memory \\ 
                              % \textit {\footnotesize{e.g.,SayPlan~\cite{rana2023sayplan}, RoboMP~\cite{lv2024robomp}, Text2Motion~\cite{lin2023text2motion}}}
                              }, color=hidden-draw, fill=myblue!40, text width=23em, text=black  
                             ]

                             % [
                             % {Action Generation with Natural Language Generation \\ \textit {\footnotesize{e.g.,RT-2~\cite{brohan2023rt}, PaLI-X~\cite{chen2023pali}, PaLM-E~\cite{driess2023palm}, OpenVLA~\cite{kim2024openvla}}}},, color=hidden-draw, fill=myblue!40, text width=27em, text=black \\
                             % ]
                       ]
                       [
                           Code Generation (\S 2.2.2), fill=myblue!60, text width=14em, text=black 
                           [
                                {Direct Code Generation  \\
                                }, color=hidden-draw, fill=myblue!40, text width=23em, text=black
                           ]
                            [
                                {Decomposition-based Generation \\
                                }, color=hidden-draw, fill=myblue!40, text width=23em, text=black
                           ]
                            [
                                {Constraint-based Generation \\
                                }, color=hidden-draw, fill=myblue!40, text width=23em, text=black
                           ]
                       ]
                       [
                              Visual Generation (\S 2.2.3), fill=myblue!60, text width=14em, text=black
                              [
                                {Video Generation Models \\
                                }, color=hidden-draw, fill=myblue!40, text width=23em, text=black
                              ]
                              [
                                {Image Generation Models \\
                                }, color=hidden-draw, fill=myblue!40, text width=23em, text=black
                              ]
                              [
                                {3D Generation Models \\
                                }, color=hidden-draw, fill=myblue!40, text width=23em, text=black
                              ]
                    
                       ]
                       [
                           State Generation (\S 2.2.4), fill=myblue!60, text width=14em, text=black
                           [
                            {Modeling observation \\
                            }, color=hidden-draw, fill=myblue!40, text width=23em, text=black
                           ]
                           [
                            {Modeling Dynamics \\
                            }, color=hidden-draw, fill=myblue!40, text width=23em, text=black
                           ]
                       ]
                ]
                [
                   Policy Layer (\S 2.3), fill=myyellow!80, text width=10em, text=black
                       [
                             Grasp Generation (\S 2.3.1), fill=myyellow!60, text width=14em, text=black
                           [
                            {Diffusion-based methods \\
                            }, color=hidden-draw, fill=myblue!40, text width=23em, text=black
                           ]
                           [
                            {VAE-based methods \\
                            }, color=hidden-draw, fill=myblue!40, text width=23em, text=black
                           ]
                           [
                            {Other generative models \\
                            }, color=hidden-draw, fill=myblue!40, text width=23em, text=black
                           ]
                       ]
                       [
                             Trajectory Generation (\S 2.3.2), fill=myyellow!60, text width=14em, text=black
                             [
                            {Sampling-based Generation \\
                            }, color=hidden-draw, fill=myblue!40, text width=23em, text=black
                           ]
                           [
                            {Large Pre-trained Model-based Generation \\
                            }, color=hidden-draw, fill=myblue!40, text width=23em, text=black
                           ]
                           [
                            {Hybrid-mode Generation \\
                            }, color=hidden-draw, fill=myblue!40, text width=23em, text=black
                           ]
                       ]
                ]
            ]   
        \end{forest}
    
    % Removed unintended closing brace or command issue
    \caption{Overview of generative models for robotic manipulation. The taxonomy shows three main categories, each with detailed sub-categories describing specific approaches and methodologies in robotic manipulation.}
    \label{fig:taxonomy}
    
\end{figure*}
